Quantum spin fluctuations and the stability of atomically-sized Bloch points

We reveal the role of the spin variables' zero-point fluctuations (ZPFs) on the stability of Bloch point (BP) singularities. As topological solitons, BPs are important in topological transitions in nanomagnets. BPs present a singularity at their core, where the long-length-scale approximation fails. We found that ZPFs bloom nearby this core, reducing the effective magnetic moment and increasing the BP's stability. As suggested by classical models, the magnonic eigenmodes found by our methods fit with the bound state of an electron surrounding a dyon, with a magnetic and an electric charge.

==> texts/100words.tex <==
Our research paper explores the impact of quantum spin fluctuations  (QSF) on the stability of Bloch point singularities. As Bloch points are important in nanomagnetism, this research sheds light on these topological solitons' unique features in the quantum regime. The study highlights the QSFs nearby the singularity at the core of Bloch points, providing systematic procedures to study the singularity's vicinity, enabling a more comprehensive understanding of the dynamics of such solitons and their role in topological transitions. We significantly contribute to the buoyant quantum magnonics and topological quantum magnetism fields. It will interest PRL's wide readership. 

==> texts/BP_Motion.tex <==
\section{Dynamical effects of The ZP field on the Bloch Point } 
We can express the effective dynamics of the Bloch point in the formalism of collective variables approach, namely, we consider the ansatz $\boldsymbol{S}(\boldsymbol{r})=\boldsymbol{S}_{0}(\hat{\mathcal{R}}(\boldsymbol{r}-\boldsymbol{X}))$ where $\boldsymbol{S}_{0}$ is the initial configuration with the symmetry axis of the BP towards the $\hat{z}$-axis,  whereas $\boldsymbol{X}=(X,Y,Z)$ is the displacement from the core of the Bloch Point, and $\boldsymbol{\Theta}=(\Theta_{x},\Theta_{y},\Theta_{z})$ being the Euler angles of the rotation axis, in such way that is valid the linear approximation $\hat{\mathcal{R}}\approx \hat{\mathbb{I}}+\boldsymbol{\Theta}\cdot \hat{L}$, where $\hat{L}_{i}$ are the generators of the rotations group $SO(3)$.  Besides, let's introduce $U(X)$ some pinning potential on the BP due to the confined geometry.  Thus, according to the Thiele approach\cite{Thiele1973, Iwasaki2013, Troncoso2014}, the Lagrangian around the equilibrium point turns out to be 
$$
L(\boldsymbol{X},\boldsymbol{\Theta})= \boldsymbol{G}_{0}\cdot (\boldsymbol{X} \times \dot{\boldsymbol{X}} )+ \Gamma_{0}\ \boldsymbol{X}\cdot \dot{\boldsymbol{\Theta}} - U(\boldsymbol{X})
$$
Here $\boldsymbol{G}_{0}$ stands for the gyrovector defined by the volumetric integral of the emergent magnetic field $(\boldsymbol{G}_{0})_{k}= \frac{\hbar S}{a^{2}}\epsilon_{ijk}\int_{V} \bn\cdot (\partial_{i}\bn\times \partial_{j}\bn)\ dV$, whereas that  $\Gamma_{0}= \frac{\hbar S}{a^{2}}S^{2}\epsilon_{ijk}\int_{V} \bn\cdot \left ( \partial_{k}\bn\times (x_{i}\partial_{j}\bn-x_{j}\partial_{i}\bn) \right )\ dV$. Note that the rest of the terms vanish because of the texture's symmetry. Hence, by means of the ansatz $\bn=(\sin(\theta)\cos(q\phi+\gamma),\sin(\theta)\sin(q\phi+\gamma),\cos(\theta))$, and the formula for the emergent magnetic field $\boldsymbol{B}_{\mathrm{emer}}=-q\ \hat{\boldsymbol{r}}/r+4\pi q\ \delta(x)\delta(y) \hat{\boldsymbol{r}}$ \cite{Elias2014}, the above integrals can be evaluated analytically in the continuum limit over a sphere of radius $R$ containing the BP, obtaining the following results $\boldsymbol{G}_{0}= \frac{8\pi\hbar S}{a^{2}} R\ \hat{\boldsymbol{z}}$ and $\Gamma_{0}= \frac{4\pi\hbar S}{3 a^{2}} R^{2}$. The Euler-Lagrange motion equations lead to the system:
\begin{align*}
\boldsymbol{G}_{0}\times\dot{X}_{i} - \Gamma_{0} \dot{\Theta}_{i} &= -\partial_{i}U(X) + f_{i} \\
\Gamma_{0} \dot{X}_{i} &= \tau_{i}
\end{align*}
On the right-hand side, we have added the force and torque $f_{i},\tau_{i}$ corresponding to the Casimir vacuum fluctuations. According to numerical evaluations of the Casimir field, we found $\boldsymbol{\tau}= \tau \hat{\boldsymbol{z}}$ .  

